Gradient flow of Einstein-Maxwell theory and Reissner-Nordstr\"om black holes

Ricci flow is a natural gradient flow of the Einstein-Hilbert action. Here we consider the analog for the Einstein-Maxwell action, which gives Ricci flow with a stress tensor contribution coupled to a Yang-Mills flow for the Maxwell field. We argue that this flow is well-posed for static spacetimes with pure electric or magnetic potentialsand show it preserves both non-extremal and extremal black hole horizons. In the latter case we find the flow of the near horizon geometry decouples from that of the exterior. The Schwarzschild black hole is an unstable fixed point of Ricci flow for static spacetimes. Here we consider flows of the Reissner-Nordstr\"om (RN) fixed point. The magnetic RN solution becomes a stable fixed point of the flow for sufficient charge. However we find that the electric RN black hole is always unstable. Numerically solving the flow starting with a spherically symmetric perturbation of a non-extremal RN solution, we find similar behaviour in the electric case to the Ricci flows of perturbed Schwarzschild, namely the horizon shrinks to a singularity in finite time or expands forever. In the magnetic case, a perturbed unstable RN solution has a similar expanding behaviour, but a perturbation that decreases the horizon size flows to a stable black hole solution rather than a singularity. For extremal RN we solve the near horizon flow for spherical symmetry exactly, and see in the electric case two unstable directions which flow to singularities in finite flow time. However, even turning these off, and fixing the near horizon geometry to be that of RN, we numerically show that the flows appear to become singular in the vicinity of its horizon.

==> Backup/magneticnearhorizon.tex <==
\subsection{Magnetic flow: Near horizon}
In the following discussion, we focus on the magnetic case. In order to do so, we consider the expression presented in \eqref{eq:magans} and write down the corresponding near horizon flow equations,
\be
T_0'(\lambda) = 2   - 2 \frac{T_0}{S_0^2}    \; , \quad S_0'(\lambda) = - 2 + \frac{2}{S_0(\lambda)}
\label{eq:horizonDEM}
\ee
The full, analytic solution to \eqref{eq:horizonDEM} gives us,
\be
\begin{split}
    S_{0}(\lambda)&=1+K_\pm(\lambda) \; ,\\
        T_{0}(\lambda)&=\frac{1+K_\pm(\lambda)\left[2\left(\lambda-\lambda_0\right)+c-\log{K_\pm(\lambda)}\right]}{1+K_\pm(\lambda)}
    \label{eq:fullmagfl}
\end{split}
\ee
where we have defined,
\be
K_\pm(\lambda) =  \mathtt{ProductLog}\left(\pm e^{-2 ( \lambda - \lambda_0 )} \right)
\ee
\textcolor{red}{
ADDED TOBY: I think the general solution is this -- so very similar to the electric case; note that $\log{K_{\pm}} = - K_{\pm} -2(\lambda - \lambda_0) - \log{\pm1}$;
\be\label{toexp}
S_0(\lambda) & = & \left(1 + K_\pm( \lambda ) \right) \nl
T_0(\lambda) & = & \frac{\left( 1 + \left( c + \frac{4(\lambda-\lambda_0)}{q^2} \right) K_\pm(\lambda) + K(\lambda)_\pm^2 \right)}{1 + K_\pm(\lambda)}
\ee
But this is actually very obvious if you look at the odes; electric case
\be
T_0'(\lambda) = 2   -  \frac{2}{T_0}    \; , \quad S_0'(\lambda) = - 2 + \frac{2 S_0(\lambda)}{T_0(\lambda)^2}
%T_0'(\lambda) = 2 e^{- 2 T_0(\lambda)}  \left( e^{T_0(\lambda)} - \phi_0^2  \right)  \; , \quad S_0'(\lambda) = - 2 + 2 \phi_0^2 S_0(\lambda) e^{-2 T_0(\lambda)} 
\label{eq:horizonDE}
\ee
and magnetic case
\be
T_0'(\lambda) = 2   - 2 \frac{T_0}{S_0^2}    \; , \quad S_0'(\lambda) = - 2 + \frac{2}{S_0(\lambda)}
\label{eq:horizonDEM}
\ee
so I think you if you take a solution to the first, the take $T \leftrightarrow S$ and $\lambda \to - \lambda$ you obviously get a solution to the second system?
}

The constant $c$ can be fixed by imposing an initial condition for $T_0$ in \eqref{eq:fullmagfl} and solving for $c$. Asymptotically as $\lambda \to \infty$ we have,
\be\label{Wdef}
K_\pm(\lambda) \to \pm e^{-2 ( \lambda - \lambda_0 )}
\ee
By taking the $+$-branch, plugging such an expression in the analytic solutions \eqref{eq:fullmagfl} and linearizing them, we are left with,
\be
\begin{split}
    S_{0}(\lambda)&=1+e^{-2 ( \lambda - \lambda_0 )} \; ,\\
        T_{0}(\lambda)&=1+e^{-2 ( \lambda - \lambda_0 )}\left[4\left(\lambda-\lambda_0\right)+c+1\right]
    \label{eq:linmagfl}
\end{split}
\ee
Introducing two new constants,
\be
a\equiv e^{2\lambda_0} \; ,\quad b\equiv c+1-4\lambda_0
\ee
the above expressions simplify as,
\be
T_0(\lambda) & = & 1 +  e^{-2 \lambda}  a  \nl
S_0(\lambda) & = & 1 +  e^{-2 \lambda} a \left( 4 \lambda  + b \right)
\label{toexp}
\ee
\begin{figure}[th]
\includegraphics[width=12cm]{Figures/GraphMF.png}
\caption{\label{analyticnh} Analytic behaviour of the near horizon magnetic flow for small perturbations around the fixed point, for $a=1$. It can be clearly observed that any displacement is brought back to $\left(S_0,T_0\right)=\left(1,1\right)$ for late flow times. The blue branch corresponds to $K_+$, while the orange one to $K_-$.
  }
\end{figure}


\newpage

\subsection{Near horizon Magnetic flow}
In the following discussion, we focus on the magnetic case. In order to do so, we consider the expression presented in \eqref{eq:magans} and write down the corresponding near horizon flow equations,
\be\label{mfnh}
T_0'(\lambda) = 2   - 2 \frac{T_0}{S_0^2}    \; , \quad S_0'(\lambda) = - 2 + \frac{2}{S_0(\lambda)}
\label{eq:horizonDEM}
\ee
In order to derive the full, analytic solution we introduce two functions,
\be
\Bar{T}_0\left(\lambda\right)\equiv S_0\left(-\lambda\right)\; ,\quad \Bar{S}_0\left(\lambda\right)\equiv T_0\left(-\lambda\right)\ .
\ee
Therefore, starting from the near horizon magnetic flow equations \eqref{mfnh}, we are left with:
\be\label{flippedeq}
\Bar{T}_0'\left(\lambda\right)=2 - \frac{2}{\Bar{T}_0} \; ,\quad \Bar{S}_0'\left(\lambda\right)=-2   + 2 \frac{\Bar{S}_0}{\Bar{T}_0^2} \ .
\ee
One can straightforwardly observe that the flow equations \eqref{flippedeq} are completely equivalent to the electric near horizon flow equations \eqref{enhf}, when $\phi_0=1$. Hence, they admit a solution of the form:
\be
\Bar{T}_0(\lambda) & = & 1 + W_\pm( \lambda )  \nl
\Bar{S}_0(\lambda) & = &  \frac{1 + \left[ c - 4(\lambda-\lambda_0) \right] W_\pm(\lambda) + W_\pm(\lambda)^2 }{1 + W_\pm(\lambda)}
\ee
where we have once more defined,
\be
W_\pm(\lambda) =  \mathtt{ProductLog}\left( \pm e^{\frac{2 ( \lambda - \lambda_0 )}{q^2}} \right)\ .
\ee
Expressing everything again in terms of $T_0$ and $S_0$, we obtain,
\be\label{fsnhm}
S_0(\lambda) & = & 1 + K_\pm( \lambda )  \nl
T_0(\lambda) & = &  \frac{1 + \left[ c + 4(\lambda-\lambda_0) \right] K_\pm(\lambda) + K_\pm(\lambda)^2 }{1 + K_\pm(\lambda)}
\ee
where the constant $\lambda_0$ was mapped to $-\lambda_0$ and the function $K_\pm$ was simply defined as,
\be
K_\pm\left(\lambda\right)\equiv W_\pm(-\lambda)=\mathtt{ProductLog}\left( \pm e^{-2 ( \lambda - \lambda_0 )} \right)\ .
\ee
In this case, we must study the asymptotic behaviour as $\lambda \to \infty$. There, we have,
\be\label{Wdef}
K_\pm(\lambda) \to \pm e^{-2 ( \lambda - \lambda_0 )}
\ee
Hence, the unstable fixed point that lies at the asymptotic past of the electric near horizon flow translates into a stable fixed point in the asymptotic future of the magnetic near horizon flow. The analysis presented in the previous section can be similarly developed for this case, producing analogous results. In particular, we can consider the fixed point $T_0=S_0=1$ and linearize the flow equations \eqref{mfnh} around it, solving them as,
\be\label{linearmnhf}
T_0\left(\lambda\right)=1+\epsilon\left(\alpha+4\beta\lambda\right)e^{-2\lambda}\ ,\quad S_0\left(\lambda\right)=1+\epsilon\beta e^{-2\lambda}\ ,
\ee
where $\epsilon\alpha$ and $\epsilon\beta$ are real parameters controlling the relevant deformations, with $|\epsilon|\ll 1$. From the exponentially dropping nature of \eqref{linearmnhf}, one can straightforwardly infer that the fixed point at $T_0=S_0=1$ is stable. Now, we can take the full solution \eqref{fsnhm} and linearize it around $\lambda\to\infty$, so that we obtain, 
\be\label{lfsnhm}
S_0(\lambda) & = & 1 \pm e^{-2 ( \lambda - \lambda_0 )}  \nl
T_0(\lambda) & = &  \left\{1 \pm\left[ c + 4(\lambda-\lambda_0) \right] e^{-2 ( \lambda - \lambda_0 )} + e^{-4 ( \lambda - \lambda_0 )}\right\} \left(1 \mp e^{-2 ( \lambda - \lambda_0 )}\right)
\ee
Choosing the positive branch, we can match $\epsilon\alpha$ and $\epsilon\beta$ with $c$ and $\lambda_0$ as,
\be
\epsilon\beta & = & e^{2\lambda_0 } \nl 
\epsilon\alpha& = & \left( c-1 - 4\lambda_0 \right) e^{2 \lambda_0 }\ .
\ee
Hence, we can phrase $c$ and $\lambda_0$ in terms of $\alpha$, $\epsilon$ and $\beta$ as:
\be
\lambda_0=\frac{1}{2}\log{\epsilon\beta}\ ,\quad c=1+\frac{\alpha}{\beta}+ 2\log{\epsilon\beta}   \ .
\ee
\begin{figure}[th]
\includegraphics[width=12cm]{Figures/MM.png}
\caption{\label{analyticnhm} Analytic behaviour of the near horizon magnetic flow for small perturbations around the fixed point. The various colors correspond to different choices for $c$ and the branches $K_{\pm}$.
  }
\end{figure}
The analytic behaviour of the near horizon flow is captured in Figure \eqref{analyticnhm}. As can be clearly observed, the sign freedom in the definition  of $K_\pm\left(\lambda\right)$ defines two distinct branches for evolutions produced by small perturbations around the fixed point. Given such a distinction, the various trajectories in the $\left(S_0,T_0\right)$ plane are then labelled by the value assigned to the relevant $c$ parameter. Being the fixed point stable, the flow always brings us back to $\left(S_0,T_0\right)=\left(1,1\right)$. The different colors correspond to different $\lambda\to-\infty$ asymptotic behaviours. Since we are actually interested in studying the flow as $\lambda$ goes to $+\infty$, there's no reason to discuss them in detail.
